A stable-compact method for qualitative properties of semilinear elliptic equations

We study the uniqueness of reaction-diffusion steady states in general domains with Dirichlet boundary data. Here we consider "positive" (monostable) reactions. We describe geometric conditions on the domain that ensure uniqueness and we provide complementary examples of nonuniqueness. Along the way, we formulate a number of open problems and conjectures. To derive our results, we develop a general framework, the stable-compact method, to study qualitative properties of nonlinear elliptic equations.

==> cg-macros.tex <==
\newcommand*{\R}{\mathbb{R}}
\providecommand*{\C}{}
\renewcommand*{\C}{\mathbb{C}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Z}{\mathbb{Z}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\T}{\mathbb{T}}
\newcommand*{\A}{\mathbb{A}}
\newcommand*{\E}{\mathbb{E}}
\newcommand*{\K}{\mathbb{K}}
\newcommand*{\F}{\mathbb{F}}
\newcommand*{\D}{\mathbb{D}}
\renewcommand*{\P}{\mathbb{P}}
\newcommand*{\e}{\mathrm{e}}
\newcommand*{\cc}{\mathrm{c}}
\newcommand*{\eps}{\varepsilon}
\newcommand*{\al}{\alpha}
\newcommand*{\Om}{\Omega}
\newcommand*{\bd}{\partial}
\newcommand*{\h}[1]{\hat{#1}}
\newcommand*{\s}[1]{\mathscr{#1}}
\newcommand*{\m}[1]{\mathcal{#1}}
\newcommand*{\f}[1]{\mathfrak{#1}}
\newcommand*{\dn}{\mathrm{d}}
\newcommand*{\diff}{\mathrm{d}}
\newcommand*{\ds}{\,\mathrm{d}}
\renewcommand*{\d}{\;\mathrm{d}}
\newcommand*{\Der}{\mathrm{D}}
\newcommand*{\der}[2]{\frac{\dn #1}{\dn #2}}
\newcommand*{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand*{\abs}[1]{\left |#1 \right|}
\newcommand*{\norm}[1]{\left \|#1 \right\|}
\newcommand*{\op}[1]{\operatorname{#1}}
\newcommand*{\sgn}{\op{sgn}}
\newcommand*{\ti}[1]{\tilde{#1}}
\newcommand*{\ubar}[1]{\underline{#1}}
\newcommand*{\tbf}[1]{\textup{\textbf{#1}}}
\newcommand*{\trm}[1]{\textup{\textrm{#1}}}
\newcommand*{\id}[1]{\op{id}_{#1}}
\newcommand*{\anon}{\,\cdot\,}
\renewcommand*{\Re}{\op{Re}}
\renewcommand*{\Im}{\op{Im}}
\newcommand*{\Ker}{\op{ker}}
\newcommand*{\Image}{\op{im}}
\newcommand*{\Span}{\op{span}}
\newcommand*{\supp}{\op{supp}}
\newcommand*{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand*{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand*{\arccot}{\op{arccot}}
\newcommand*{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand*{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand*{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand*{\MLoc}{\m M_{c,\text{loc}}}
\newcommand*{\BM}{Brownian motion~}
\renewcommand*{\And}{\quad \textrm{and} \quad}
\newcommand*{\For}{\quad \textrm{for }}
\newcommand*{\ForAll}{\quad \textrm{for all }}
\newcommand*{\nab}{\nabla}
\newcommand*{\trdeg}{\op{tr\,deg}}
\newcommand*{\gr}{\op{gr}}
\newcommand*{\rees}{\op{Rees}}
\newcommand*{\Spec}{\op{Spec}}
\renewcommand*{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand*{\div}{\op{div}}
\newcommand*{\bbraket}[1]{\left \langle \! \left \langle #1 \right \rangle \! \right \rangle}
\newcommand*{\power}[1]{{#1}[\![X]\!]}
\newcommand*{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\newcommand*{\mr}{\mathring}
\newcommand*{\smallO}{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}%
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%
  }

\newcommand*{\iu}{\mathrm{i}}

\newcommand*{\smallbar}[1]{\overline{#1}}
\let\temp\bar
\let\bar\smallbar
\let\smallbar\temp
\let\temp\undefined

\newcommand*{\Hu}{\mathbb{H}}
\let\temp\H
\let\H\Hu
\let\Hu\temp
\let\temp\undefined

\newcommand*{\deep}[2][\Omega]{#1[#2]}
